Generalised functional additive mixed models with compositional covariates for areal Covid-19 incidence curves

We extend the generalised functional additive mixed model to include (functional) compositional covariates carrying relative information of a whole. Relying on the isometric isomorphism of the Bayes Hilbert space of probability densities with a subspace of the $L^2$, we include functional compositions as transformed functional covariates with constrained effect function. The extended model allows for the estimation of linear, nonlinear and time-varying effects of scalar and functional covariates, as well as (correlated) functional random effects, in addition to the compositional effects. We use the model to estimate the effect of the age, sex and smoking (functional) composition of the population on regional Covid-19 incidence data for Spain, while accounting for climatological and socio-demographic covariate effects and spatial correlation.

==> latexmkrc <==
# HACK: this width seems to change with every compile, so
# latexmk runs latex too many times; ignore it
$hash_calc_ignore_pattern{'aux'} = 'statsocwidth';

# All the other default settings on Overleaf
# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}
